An Efficient Decomposition Framework for Discriminative Segmentation with Supermodular Losses

Several supermodular losses have been shown to improve the perceptual quality of image segmentation in a discriminative framework such as a structured output support vector machine (SVM). These loss functions do not necessarily have the same structure as the one used by the segmentation inference algorithm, and in general, we may have to resort to generic submodular minimization algorithms for loss augmented inference. Although these come with polynomial time guarantees, they are not practical to apply to image scale data. Many supermodular losses come with strong optimization guarantees, but are not readily incorporated in a loss augmented graph cuts procedure. This motivates our strategy of employing the alternating direction method of multipliers (ADMM) decomposition for loss augmented inference. In doing so, we create a new API for the structured SVM that separates the maximum a posteriori (MAP) inference of the model from the loss augmentation during training. In this way, we gain computational efficiency, making new choices of loss functions practical for the first time, while simultaneously making the inference algorithm employed during training closer to the test time procedure. We show improvement both in accuracy and computational performance on the Microsoft Research Grabcut database and a brain structure segmentation task, empirically validating the use of several supermodular loss functions during training, and the improved computational properties of the proposed ADMM approach over the Fujishige-Wolfe minimum norm point algorithm.

==> nonsupermodular.tex <==
We show in detail how the presence of $\gamma$ in Equation~\eqref{eq:supermodularLoss} removes the submodularity guarantee. Given the loss augmented inference in Equation~\eqref{eq:maxenergy} with the joint feature function in Equation~\eqref{eq:feature}, as well as our supermodular loss in Equation~\eqref{eq:supermodularLoss}, we can expand Equation~\eqref{eq:maxenergy} as:
\begin{align}
&\arg\min_{\tilde{y}}\ - \langle \begin{pmatrix} w_u\\w_p \end{pmatrix}, 
\begin{pmatrix} \sum_{j=1}^{p} \phi_u(x,y^{j}) \\ \sum_{(k,l) \in \mathcal{E}} \phi_p(x,y^{k},y^{l}) \end{pmatrix} \rangle 
- \Delta(y,\tilde{y})
\end{align} 
Denote $E_u$ the unary potential, $E_p$ the pairwise potential for  this loss augmented inference. Here we try to write the problem as one graph cut problem. First we have the combined unary potential:
\begin{equation}
E_u(y^j) = - \langle w_u, \phi_u(x,y^j ) \rangle -  [y^{j} \neq \tilde{y}^j].
\end{equation}
Then we have the combined pairwise potential as in Equation~\eqref{eq:combinedLossPairwiseEnergy} where $\odot$ is the Hadamard product.
In the second term of $E_p(y^k,y^l)$, the existence of $\gamma$ removes the guarantee of the submodularity of this minimization problem: $w_{00}+w_{11}\geq w_{01}-w_{10}$ is guaranteed, but we may arbitrarily add or subtract $\gamma$ from either side of the inequality according to Equation~\eqref{eq:combinedLossPairwiseEnergy}, for different cases of the ground truth edge $(y^{k}, y^{l})$. This is exactly due to the fact that the loss function maps to a set function by considering the set of misperdicted pixels, while the inference maps to a set function by considering the set of pixels that are labeled as foreground, which are two different mappings.

\begin{strip}
\begin{align}
& E_p(y^k,y^l)  = - \begin{pmatrix} w_{00} & w_{01}\\w_{10} & w_{11} \end{pmatrix}  \odot 
 \begin{pmatrix} [y^{k} = y^{l} = -1]  & [\tilde{y}^{k} =-1 \wedge \tilde{y}^{l}=+1] \\ [y^{k} =+1 \wedge  y^{l}=-1]  & [\tilde{y}^{k} = \tilde{y}^{l} = +1]  \end{pmatrix} \nonumber \\
 & - \gamma\times \begin{pmatrix} [(y^{k} = y^{l} = -1) \wedge (\tilde{y}^{k} = \tilde{y}^{l} = +1) ]  & [(y^{k} =-1 \wedge y^{l}=+1)  \wedge (\tilde{y}^{k} =+1 \wedge \tilde{y}^{l}=-1) ] \\ [(y^{k} =+1 \wedge  y^{l}=-1) \wedge (\tilde{y}^{k} =-1 \wedge \tilde{y}^{l}=+1) ]  & [(y^{k} = y^{l} = +1) \wedge (\tilde{y}^{k} = \tilde{y}^{l} = -1)]  \end{pmatrix} \label{eq:combinedLossPairwiseEnergy} 
\end{align}
\end{strip}

